Bayesian Bi-level Sparse Group Regressions for Macroeconomic Density Forecasting

We propose a Machine Learning approach for optimal macroeconomic density forecasting in a high-dimensional setting where the underlying model exhibits a known group structure. Our approach is general enough to encompass specific forecasting models featuring either many covariates, or unknown nonlinearities, or series sampled at different frequencies. By relying on the novel concept of bi-level sparsity in time-series econometrics, we construct density forecasts based on a prior that induces sparsity both at the group level and within groups. We demonstrate the consistency of both posterior and predictive distributions. We show that the posterior distribution contracts at the minimax-optimal rate and, asymptotically, puts mass on a set that includes the support of the model. Our theory allows for correlation between groups, while predictors in the same group can be characterized by strong covariation as well as common characteristics and patterns. Finite sample performance is illustrated through comprehensive Monte Carlo experiments and a real-data nowcasting exercise of the US GDP growth rate.

==> inputs/Prior_additional_elements.tex <==
%================================================================================================================================================================================================
\input{inputs/Appendix_prior_short}
%================================================================================================================================================================================================
\subsection*{Induced prior on $\varphi_j$}\label{A:sss:prior_varphi}
\indent The prior \eqref{eq:prior:dirac}-\eqref{eq:prior:b} induces a conditional prior on the random function $\varphi_j$, given $\{v_{ji}\}_{i=1}^g$ and $g$, which can be viewed as a mixture of a degenerate Gaussian process and a Dirac distribution at zero. To see this, denote $z_{j,t-h,i} := z_{ji}(\bx_{j,t-h})$ and let $\Omega_{0,j}:\mathcal{H}_j\rightarrow \mathcal{H}_j$ be a covariance operator defined as: $\forall h\in\mathcal{H}_j$, $(\Omega_{0,j}h)(\cdot) := \sum_{i=1}^g v_{ji}^2 \langle z_{ji},h \rangle z_{ji}(\cdot)$, where $\langle\cdot,\cdot\rangle$ is the inner product in $\mathcal{H}_j$. If $\mathcal{H}_j$ is an infinite dimensional space, or has dimension larger than $g$, then $\Omega_{0,j}$ is not injective and has a nontrivial null space that contains $B_{t,j}(g)$. Hence, \eqref{eq:prior:dirac}-\eqref{eq:prior:b} induce the following conditional mixture prior on the random function $\varphi_j$: for every $j\in\{1,\ldots,N\}$,
\begin{equation}
  \varphi_j|\pi_0, \{v_{ji}\}_{i=1}^g, g \sim (1 - \pi_0)\mathcal{GP}(0,\Omega_{0,j}) + \pi_0 \delta_0(\varphi_j).
\end{equation}
As $g\rightarrow \infty$, the $\mathcal{GP}(0,\Omega_{0,j})$ is a well-defined Gaussian Process in $\mathcal{H}_j$ if and only if $\Omega_{0,j}$ is a trace-class operator, that is, if $\lim_{g\rightarrow\infty}\sum_{i=1}^g v_{ji}^2 <\infty$ by assuming $\{z_{ji}\}_i$ forms an orthonormal system. Once we integrate out $v_{ji}^2$ with respect to its prior, we find that $\EE[v_{ji}^2] =\EE[\EE[v_{ji}^2|\tau_j, \pi_1]] = 3d_1\lambda_{1,j}^2/[4(c_1 + d_1)]$. So, $\Omega_{0,j}$ is a trace-class operator if $3d_1\lambda_{1,j}^2/[4(c_1 + d_1)] = \mathcal{O}(1/g)$, which is guaranteed by Assumption \ref{Ass:3} \textit{(iv)} in the main document.%\\
%================================================================================================================================================================================================
\subsection*{Modified priors}
It is worth noting that some priors defined in Section \ref{sec:priors} can be slightly, but conveniently, modified without affecting the theoretical properties discussed in Section \ref{sec:Asymptotic_Analysis}. For instance, we can allow $\pi_{1}$, which controls for the overall prior inclusion probability for the groups of coefficients, to be group-specific. In this case, we can replace $\pi_{1}$ in step \textit{(b-1)} of Algorithm 1%\ref{algorithm:1} 
with $\pi_{1,j}$, and change the conditional posterior of $\pi_{1}$ in step \textit{(e)} with:
\begin{displaymath}
\pi_{1,j} \vert \textit{rest} \sim \mathcal{B}\left(g-\sum_{i=1}^{g}\gamma_{1,ji}+c_{1},\sum_{i=1}^{g}\gamma_{1,ji}+d_{1} \right).
\end{displaymath}
Further, we can employ a hierarchical prior for the variance of the error distribution, as in \citet{Bitto2019}: $\sigma^{2}\vert a_{1} \sim \mathcal{G}^{-1} (a_{0},a_{1})$, $a_{1}\sim\mathcal{G}(e_{0},e_{1})$,
%\begin{displaymath}
%\sigma^{2}\vert a_{1} \sim \mathcal{G}^{-1} (a_{0},a_{1}) \qquad\qquad a_{1}\sim\mathcal{G}(e_{0},e_{1})
%\end{displaymath}
with hyperparameters $a_{0}$, $e_{0}$, and $e_{1}$, set to conventional values $a_{0}=2.5$, $e_{0}=5$, $e_{1}=e_{0}/(a_{0}-1)$. In this case, we extend step \textit{(a)} with the conditional posterior distribution of $a_{1}$:
\begin{displaymath}
a_{1} \vert \textit{rest} \sim \mathcal{G}\left(e_{0}+a_{0}, e_{1}+\frac{1}{\sigma^{2}}\right).
\end{displaymath}
Preliminary analysis pointed to an improvement, although marginal, of estimation results when these changes are accounted for in the MCMC sampling scheme. The modified priors are hence implemented in Algorithm 1 %\ref{algorithm:1} 
for the remainder of the paper. 
%================================================================================================================================================================================================
\subsection*{Choice of hyperparameters for implementation}
In the Monte Carlo analysis reported in Section \ref{sec:MCsim} and in the empirical application reported in Section \ref{sec:emp_app}, the hyperparameters $\lambda_{0}$ and $\lambda_{1,j}$ of the prior for $\tau_j$ are set to $\lambda_{0}=1/2$ and $\lambda_{1,j}=\log(\log(\max(N,T)))$. Both satisfy the conditions in our theoretical analysis, but other values are also compatible with our theory.
As for the hyperparameters of the priors on $\pi_{0}$ and $\pi_{1}$, their values must be chosen very carefully, as they control the overall amount of between-group and within-group prior sparsity. Assumption \ref{Ass:3} and Appendix \ref{App:hyperparam} provide conditions and guidelines for the choice of these hyperparameters. By fixing $d_{0}=d_{1}=1$, then Assumption \ref{Ass:3} \textit{(i)} - \textit{(ii)} implies that $c_{0}$ and $c_{1}$ have to satisfy the following lower-bounds: for every $N>1$,
\begin{equation}\label{eq:lower_bounds}
  c_0 \geq 1 -N + \frac{N^{u_0+1}}{k_0}, \qquad\qquad c_1 \geq 1 - Ng + \frac{(s_0^{gr}g)^{u_1} Ng}{k_1},
\end{equation}
\noindent where $k_0$ and $k_1$ are constants, and $u_0$ and $u_1$ have to belong to intervals whose bounds depend on DGP parameters $(N,s_{0}^{gr},s_{0},g)$. The non-asymptotic lower-bounds in \eqref{eq:lower_bounds} are useful in practice if optimal values for $c_0$ and $c_1$ are selected through a grid search. %given these lower-bounds, a data-driven approach can be used to fine-tune the optimal parameters.
In this paper, we propose to select $c_0$ and $c_1$ by using a data-driven approach based on the Deviance Information Criterion (DIC; \citealp{Spiegelhalter2002}), defined as:
\begin{equation}\label{eq:DIC}
\text{DIC}(\mathbf{c}|y,\bX) := -4 \mathbb{E}_{\boldsymbol\btheta,\sigma^2}\big[\log f(y\vert \boldsymbol\btheta,\sigma^2,\bX)\vert y,\bX, \mathbf{c} \big] + 2\log f(y\vert \widehat{\btheta}_{\mathbf{c}},\widehat\sigma_{\mathbf{c}}^2,\bX),
\end{equation}
where $(\btheta^{\prime}_{\mathbf{c}},\sigma^{2}_{\mathbf{c}})^{\prime}$ denotes the model parameters for a given set of hyperparameters $\mathbf{c}=(c_{0},c_{1})$, and $(\widehat{\btheta}_{\mathbf{c}},\widehat\sigma_{\mathbf{c}}^2)$ is a point estimate of $(\btheta^{\prime}_{\mathbf{c}},\sigma^{2}_{\mathbf{c}})^{\prime}$.\footnote{The first part of \eqref{eq:DIC} is the posterior mean deviance, which is here estimated by averaging the log-likelihood function, $\log  f(y\vert \btheta,\sigma^2,\bX)$, over the posterior draws of $(\btheta,\sigma^2)$. $(\widehat{\btheta}_{\mathbf{c}},\widehat\sigma_{\mathbf{c}}^2)$ is computed using the posterior median for $\btheta$ and the posterior mean for $\sigma^2$.}
This metrics of fit presents the advantage of being easily available from the Gibbs output, with no additional costs in terms of computational burden. We hence select the hyperparameters $c_{0}$ and $c_{1}$ that minimize the DIC by performing a random search on a fine 2-dimensional grid, with lower-bounds set as described in \eqref{eq:lower_bounds}. In the Monte Carlo simulations, we set the lower-bounds at the largest possible value over all the alternative DGPs considered. In this way we ensure that the selected $c_0$ and $c_1$ satisfy \eqref{eq:lower_bounds} for all the DGPs under comparison. In empirical applications, $s_{0}^{gr}$ and $s_{0}$ are unknown, but we recommend to tune them at some arbitrary values such that the inequalities in \eqref{eq:lower_bounds} are satisfied for low values of $c_{0}$ and $c_{1}$. Therefore, the price to pay for not knowing $s_{0}^{gr}$ and $s_{0}$ is simply to have to search on a larger grid. As an alternative to the DIC, one could select $c_0$ and $c_1$ by using marginal likelihood approaches \citep{Chib1995,ChibJeliazkov2001}, which are often considered in the literature for model comparison (\textit{e.g.}, Bayes factor). Our experience in our particular setting has pointed out in favour of the DIC.


==> inputs/introduction_long.tex <==
Forecast of macroeconomic aggregates has been increasingly resorting to machine-learning-based methods and to large datasets released by official or alternative sources. These datasets might be challenging to handle because of their large dimension compared to the number of available observations in the time dimension. On the other hand, the variables in these datasets are often organised in groups which can help in reducing the dimensionality. How to optimally exploit this group-structure to make inference has been little explored in the econometric forecasting literature and the few existing theoretical contributions are limited to point forecast. This paper provides the development of a comprehensive inference procedure that, in addition to provide parameter recovery and point forecast, also provides uncertainty assessments and density forecast. Importantly, our machine-learning procedure is fully interpretable, which is crucial for the policy makers that wants to exploit. In this high-dimension with group-structure framework, we address three questions: \textit{(i)} optimality: how can we construct optimal forecasts? \textit{(ii)} interpretability: how can we detect the relevant driving factors? and \textit{(iii)} flexibility: how can we allow for nonlinearities and mixed frequencies?

Groups might be formed by predictors that present strong covariation, common characteristics and patterns. Some datasets may be organised in groups by the researcher according to economic criteria. For example, real economic activity can be analysed by using a large number of official series arranged in homogeneous blocks of indicators, such as production, employment, consumption, and housing (see \textit{e.g.} \citealp{MoenchNgPotter2013} and \citealp{McCracken2016}). Other datasets may be organised in a group structure directly by the data provider. This is the case, for instance, of the Google Search data used in \cite{FerraraSimoniJBES}. From the point of view of the policymaker, a desirable forecasting model should provide accurate predictions as well as interpretable results. Once the predictors have been grouped, interpretability can be achieved by detecting the relevant driving factors within these groups.

In this paper, we assume that the group structure is given and we are interested in how to take advantage of this feature to reduce a potentially large dimensionality. We therefore extend the concept of sparsity to the group structure by assuming that the model is bi-level sparse, \textit{i.e.} sparse at the group level and within groups. This means that some groups and some predictors within each group are irrelevant for modelling and forecasting the target variable, conditional on the remaining predictors. Since the inspiring work of \citet{Simon2013}, who introduced a shrinkage operator combining the Lasso at the variable level and the Group Lasso at the group level (the Sparse Group Lasso, SGL), the literature has increasingly focused on bi-level sparse recovery in a relatively high-dimensional framework. For instance, \citet{Huang2012} and \citet{Breheny2015} replaced the Lasso-type penalties in the SGL with alternative operators, such as the Smoothly Clipped Absolute Deviation (SCAD), the Minimax Concave Penalty (MCP), and the Exponential Penalty (EP). \citet{Xu2015} derived a Bayesian version of the SGL as well a sparse group selection approach based on a bi-level spike-and-slab prior. \citet{ChenChuYuanWu2016} proposed a similar sparse group selection prior, although their sampling approach is substantially different from the one in \citet{Xu2015}. Recently, \cite{Babii2022} studied the SGL for point forecast in a Mixed Data Sampling (MIDAS) framework.

Building on this literature, our paper extends exact bi-level sparsity to general time-series forecasting models and widens the relevance of group structure beyond datasets organised in groups as described above. Indeed, the general model we consider is flexible enough to include, in addition to linear regression models with many predictors organised in groups, MIDAS regression models where the weighting function of the high-frequency lag polynomial is nonparametric, and nonlinear forecasting models as special cases. These nonparametric models are suitable for capturing complex relationships between the target variable and the predictors. The group structure arises because for each predictor there is a nonparametric function to be estimated that we write through a generalized Fourier expansion and the elements of this expansion are the elements of one group. Depending on the model, the nonparametric function can be a function of the high-frequency lagged period (for MIDAS), a function of one predictor, or a function of interactions among predictors. Each nonparametric function is then approximated by truncating the generalised Fourier series at some threshold $g\geq 1$. Thus, while the true model is allowed to have an infinite number of elements in each group, we work with an approximated model that restricts each group to no more than $g\geq 1$ components. This introduces a bias that vanishes asymptotically as $g$ increases with the sample size $T$. The approximated model exhibits a bi-level sparsity: at the group level, only $s_0^{gr}$ groups among the $N$ groups are active, and within each active group, only a few elements have a non-zero impact on the target variable. Importantly, we allow for both $N$ and $g$ to be large compared to $T$.

For estimation and selection purposes, we adopt a Bayesian method based on a hierarchical prior that induces bi-level sparsity. Bayesian procedures have shown to be attractive for forecasting and nowcasting when the number of parameters to estimate is large compared to the sample size (see \textit{e.g.} \citealp{BanburaGiannoneReichlin2010}). They provide a built-in prediction with optimal properties and supply uncertainty quantification automatically which is not the case for frequentist procedures. In the present framework, the Bayesian analysis requires to elicit a prior that charges only the approximated model and is able to generate a group structure with bi-level sparsity. We propose a prior that models the coefficients of each block of predictors independently conditional on common hyperparameters. After marginalization, the coefficients in each group become correlated in the prior. Our hierarchical prior consists of two mixture distributions -- one for the parameters at the group level and one for the parameters within each group -- that are defined as a two-components mixtures between a continuous distribution (respectively, Normal and half-Normal) and a Dirac distribution with mass one at zero. The latter induces exact zeros for the coefficients with non-negligible probability. The hyperparameters of the Normal and half-Normal distributions, as well as the weights of the mixtures and the model variance, are endowed with prior distributions.

Compared to the existing literature, a number of new features are introduced in this paper. First, the proposed method does not require orthogonality between the groups of covariates, such that cross-correlation between variables located in different groups is allowed by our theory. Second, the proposed prior is closely inspired by \citet[Section 3.2]{Xu2015}, with nominal minor modifications. However, we show that these modifications yield a posterior distribution with good frequentist asymptotic properties. Third, we establish optimal frequentist theoretical properties of our Bayesian procedure in a setting where the true data generation process (DGP) has a bi-level sparse group structure. Asymptotic properties are then established for the sample size $T$ increasing to infinity and for the number of groups $N$, the number of active groups $s_0^{gr}$, the number of components per groups $g$, and the number of active predictors in the model $s_0$ increasing to infinity with $T$. We recover the contraction rate of the posterior distribution of the parameters of interest and of the in-sample prediction. Remarkably, our posterior contraction rate attains the minimax rate established in \cite{Cai2022IEEE} and in \cite{LiZhangYin2022} under mild conditions on the prior and the DGP. In particular, the rate of contraction is faster than the rate obtained without exploiting the group structure. We also analyse the convergence of the posterior mean estimator. Further, the optimal forecast is constructed by using the posterior predictive distribution, which is well-known to dominate plug-in predictive distributions when there is prior information. The posterior predictive is shown to be consistent. Finally, the proposed prior is computationally convenient, as it relies on a relatively simple Gibbs sampler with one Metropolis-Hasting step to simulate from the posterior distribution. In particular, its computational advantage is particularly strong with respect to the prior proposed by \citet{ChenChuYuanWu2016}.

The present paper significantly departs in several important ways from our previous work \citep{MoglianiSimoni2021}, where sparsity only at the group level was assumed. For instance, we consider here a generally nonparametric model that nests the MIDAS regression as a special case, while \citet{MoglianiSimoni2021} only focus on MIDAS regression models. Most importantly, compared to the group sparsity assumption, the bi-level sparsity assumption substantially changes the rate of contraction of the posterior distribution and the structure of the proofs provided in \citet{MoglianiSimoni2021}. The main drawback of assuming group sparsity, instead of bi-level group sparsity, when the true model is bi-level sparse is that the posterior does not put zero mass asymptotically on models with dense groups. Therefore, if the true model is bi-level sparse, then the posterior obtained under group sparsity only is not ensured to recover the correct sparsity pattern, implying also a worsening of out-of-sample predictive accuracy. We show this in our first Monte Carlo simulation, where the selection results obtained by the prior introduced in the present paper is compared with those from the sparse Group Lasso prior proposed by \cite{MoglianiSimoni2021}. We further show that the results are robust to a number of alternative features in the DGP, such as sophisticated within- and between-groups correlation structures and asymmetric shocks.

Our second Monte Carlo experiment focuses on a DGP accommodating mixed-frequency data, where we allow for nonparametric weighting functions (for each high-frequency predictor) which we write as truncated generalized Fourier series. We find good performance in sparse settings with a parsimonious number of active high-frequency variables. %{\dr can we say that the results here are better than in our previous paper?}
Unlike other shrinkage priors, our approach allows for a flexible treatment of the error term. We show that only a slight modification of the proposed prior is required to account for stochastic volatility and ARMA errors \citep{Chan2014,Zhang2020}. These features may be relevant in some macroeconomic applications \citep{CCMM} and can be straightforwardly accommodated in our framework.

Finally, we illustrate our approach in an empirical application on nowcasting the US quarter-on-quarter GDP growth rate with 122 indicators sampled at monthly frequencies and extracted from FRED-MD \citep{McCracken2016}. We show that our prior provides good nowcasting performance (in terms of point and density forecast) when compared to the benchmark AR(1) and the Bayesian Sparse Group Lasso \citep{Xu2015}.

The paper is structured as follows. In Sections \ref{sec:model} and \ref{sec:priors} we present respectively the model and the prior. The asymptotic properties of our procedure are analysed in Section \ref{sec:Asymptotic_Analysis}. The Gibbs sampler and the computational aspects are presented in Section \ref{sec:MCMC}, while the results of the Monte Carlo experiments are discussed in Section \ref{sec:MCsim}. Section \ref{sec:emp_app} provides an empirical application on nowcasting U.S. GDP growth. Finally, Section \ref{sec:conclusions} concludes. The proofs for the main theoretical results are provided in Appendix \ref{App:main}, while the remaining proofs are provided in an Online Appendix.

